Spatial-Temporal Identity: A Simple yet Effective Baseline for Multivariate Time Series Forecasting

Multivariate Time Series (MTS) forecasting plays a vital role in a wide range of applications. Recently, Spatial-Temporal Graph Neural Networks (STGNNs) have become increasingly popular MTS forecasting methods due to their state-of-the-art performance. However, recent works are becoming more sophisticated with limited performance improvements. This phenomenon motivates us to explore the critical factors of MTS forecasting and design a model that is as powerful as STGNNs, but more concise and efficient. In this paper, we identify the indistinguishability of samples in both spatial and temporal dimensions as a key bottleneck, and propose a simple yet effective baseline for MTS forecasting by attaching Spatial and Temporal IDentity information (STID), which achieves the best performance and efficiency simultaneously based on simple Multi-Layer Perceptrons (MLPs). These results suggest that we can design efficient and effective models as long as they solve the indistinguishability of samples, without being limited to STGNNs.

==> Sections/RelatedWork.tex <==
\section{Related Work}
\subsection{Spatial-Temporal Graph Neural Networks}
The accuracy of multivariate time series forecasting has been largely improved by artificial intelligence~\cite{Innovation}, especially deep learning techniques.
Among these techniques, Spatial-Temporal Graph Neural Networks~(STGNNs) are the most promising methods, 
which combine Graph Neural Networks (GNNs)~\cite{2017GCN, 2016ChebNet} and sequential models~\cite{2014GRU, FC-LSTM} to model the spatial and temporal dependency jointly.
Graph WaveNet~\cite{GWNet}, MTGNN~\cite{2020MTGNN}, STGCN~\cite{2018STGCN}, and StemGNN~\cite{2020StemGNN} combine graph convolutional networks and gated temporal convolutional networks with their variants. These methods are based on convolution operation, which facilitates parallel computation.
DCRNN~\cite{2017DCRNN}, ST-MetaNet~\cite{2019STMetaNet}, AGCRN~\cite{2020AdaptiveGCRN}, and TGCN~\cite{2019TGCN} combine diffusion convolutional networks and recurrent neural networks~\cite{2014GRU, FC-LSTM} with their variants. 
They follow the seq2seq~\cite{2014Seq2Seq} architecture to predict step by step.
Moreover, attention mechanism is widely used in many methods, such as GMAN~\cite{2020GMAN} and ASTGCN~\cite{2019ASTGCN}. 
Although STGNNs have made significant progress, the complexity of STGNNs is high because it needs to deal with both temporal and spatial dependency at every step.
Therefore, STGNNs can only take short-term historical time series as input, such as the past 1 hour~(twelve time steps in many datasets).

More recently, an increasing number of works~\cite{2018NRI, 2019LDS, 2021GTS} have focused on joint learning of graph structures and graph neural networks to model the dependencies between nodes~(\ie time series in our work).
% NRI~\cite{2018NRI} takes the form of a variational auto-encoder, in which the latent code represents the underlying dependency graph and the reconstruction is based on graph neural networks.
LDS~\cite{2019LDS} models the edges as random variables whose parameters are treated as hyperparameters in a bilevel learning framework.
The random variables parameterize the element-wise Bernoulli distribution from which the adjacency matrix $\mathbf{A}$ is sampled.
GTS~\cite{2021GTS} introduces a neighborhood graph as a regularization that improves graph quality and reformulates the problem as a unilevel optimization problem.
Notably, We follow the framework of GTS but enhance it by the pre-training model since TSFormer gives better latent representations of time series for calculating their correlations.
% We will conduct the ablation studies in Section {\color{red}X}.

% GWNet MTGNN STGCN 2020StemGNN
% DCRNN STMetaNet 2020AdaptiveGCRN 2019TGCN
% GMAN 
% FCGAGA 2021HGCN

% Spatial Temporal Graph Neural Networks: DCRNN, GWNet, MTGNN, ASTGCN, STGCN, GMAN, 2020StemGNN. FCGAGA, 2020AdaptiveGCRN, 2021HGCN, 2019STMetaNet, 2019TGCN, Innovation, GCN
% Graph Stucture Learning: NRI, LDS, GTS, 2021REST
% 结论：取得了很大的进展，但是由于复杂度的限制，只能应用在短期序列上；
\subsection{Pre-training Model}
% NLP
The pre-training model is used to learn a good representation from massive unlabeled data and then use these representations for other downstream tasks.
Recent studies have demonstrated significant performance gains on many natural language processing tasks with the help of the representation extracted from pre-training models~\cite{2020PTM}.
Prominent examples are the BERT~\cite{2019BERT} and GPT~\cite{2020GPT}, which are based on the Transformer encoder and decoder, respectively.
The Transformer architecture is more powerful and more efficient than LSTM architecture~\cite{FC-LSTM, 2018ELMO} and has become the mainstream approach for designing pre-training models.
% CV
More recently, Transformer for images has attracted increasing attention because of its powerful performance.
ViT~\cite{2020ViT} proposes to split an image into patches and provide the sequence of linear embeddings of these patches as an input to a Transformer, showing impressive performance.
However, ViT needs supervised training, which requires massive labeled data.
On the contrary, MAE~\cite{2021MAE} uses self-supervised learning based on the masked autoencoding strategy. 
MAE enables us to train large models efficiently and effectively and outperforms supervised pre-training.
Although the pre-training model has made significant progress in natural language processing and computer vision, progress in time series lags behind them. In this paper, we propose a pre-training model~(named TSFormer) for time series based on Transformer blocks and improve the performance of the downstream forecasting task.


==> Sections/Visualization.tex <==
\subsection{Visualization}
% \section{Visualization}
\label{appendix_visualization}
In order to further intuitively understand and evaluate our model, in this section, we give more visualizations.
First, we provide more visualizations about reconstructions of the TSFormer on PEMS04 dataset like Figure \ref{inspecting}(b).
The results are shown in Figure \ref{vis_rec}. 
Note that due to space limitation, we only visualize time series in a small window rather than the whole input time series $\mathbf{S}^i$.
% We are surprisingly find that even given very limited information surrounding the unmasked patches, TSFormer reconstructs the masked patches very accurately.
Surprisingly, we find that even given very limited information surrounding the unmasked patches, TSFormer reconstructs the masked patches accurately.
These results again indicate that our model has a strong ability to learn rich temporal patterns from very long-term time series.
Then, we visualize the prediction of our model and the groundtruth data based on METR-LA dataset.
We randomly selected six time series and displayed their data from June 13th 2012 to June 16th 2012~(located the test dataset).
The forecasting results on six randomly selected time series are shown in Figure \ref{vis_for}.
We can see that our model can accurately make predictions for different time series.
Furthermore, we find that the model has the ability to resist noise. 
For example, in the right top figure, the traffic sensor apparently failed in the afternoon of June 13th, 2012. 
However, the model does not overfit the noise.

\begin{figure}[ht]
    % \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
  \centering
  \includegraphics[width=1\linewidth]{Figures/Vis_Reconstruction_2.pdf}
  \caption{Reconstruction visualizations.}
  \label{vis_rec}
\end{figure}

\begin{figure}[ht]
    % \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
  \centering
  \includegraphics[width=1\linewidth]{Figures/Vis_Forecasting_2.pdf}
  \caption{Forecasting visualizations.}
  \label{vis_for}
\end{figure}

